Algorithmic Fairness from a Non-ideal Perspective

Inspired by recent breakthroughs in predictive modeling, practitioners in both industry and government have turned to machine learning with hopes of operationalizing predictions to drive automated decisions. Unfortunately, many social desiderata concerning consequential decisions, such as justice or fairness, have no natural formulation within a purely predictive framework. In efforts to mitigate these problems, researchers have proposed a variety of metrics for quantifying deviations from various statistical parities that we might expect to observe in a fair world and offered a variety of algorithms in attempts to satisfy subsets of these parities or to trade off the degree to which they are satisfied against utility. In this paper, we connect this approach to \emph{fair machine learning} to the literature on ideal and non-ideal methodological approaches in political philosophy. The ideal approach requires positing the principles according to which a just world would operate. In the most straightforward application of ideal theory, one supports a proposed policy by arguing that it closes a discrepancy between the real and the perfectly just world. However, by failing to account for the mechanisms by which our non-ideal world arose, the responsibilities of various decision-makers, and the impacts of proposed policies, naive applications of ideal thinking can lead to misguided interventions. In this paper, we demonstrate a connection between the fair machine learning literature and the ideal approach in political philosophy, and argue that the increasingly apparent shortcomings of proposed fair machine learning algorithms reflect broader troubles faced by the ideal approach. We conclude with a critical discussion of the harms of misguided solutions, a reinterpretation of impossibility results, and directions for future research.

==> oldrefs.tex <==
@book{Anderson2010,
address = {Princeton},
author = {Anderson, Elizabeth},
publisher = {Princeton University Press},
title = {{The Imperative of Integration}},
year = {2010}
}

@article{Angwin2016,
author = {Angwin, Julia and Larson, Jeff and Mattu, Surya and Kirchner, Lauren},
journal = {ProPublica},
title = {{Machine bias: There's software used across the country to predict future criminals. And it's biased against blacks}},
year = {2016}
}

@inproceedings{Barabas2018,
  author    = {Chelsea Barabas and
               Madars Virza and
               Karthik Dinakar and
               Joichi Ito and
               Jonathan Zittrain},
  title     = {Interventions over Predictions: Reframing the Ethical Debate for Actuarial
               Risk Assessment},
  booktitle = {Conference on Fairness, Accountability and Transparency, {FAT} 2018,
               23-24 February 2018, New York, NY, {USA}},
  pages     = {62--76},
  year      = {2018}
}

@article{Barocas2016,
author = {Barocas, Solon and Selbst, Andrew D.},
journal = {California Law Review},
number = {3},
pages = {671--732},
title = {{Big Data's Disparate Impact}},
volume = {104},
year = {2016}
}

@article{Bear2011a,
author = {Bear, Julia B and Woolley, Anita Williams},
doi = {10.1179/030801811X13013181961473},
isbn = {03080188},
journal = {Interdisciplinary Science Reviews},
number = {2},
pages = {146--153},
title = {{The role of gender in team collaboration and performance}},
volume = {36},
year = {2011}
}

@article{Berk2018,
author = {Berk, Richard and Heidari, Hoda and Jabbari, Shahin and Kearns, Michael and Roth, Aaron},
doi = {10.1177/0049124118782533},
journal = {Sociological Methods {\&} Research},
keywords = {criminal justice,discrimination,fairness,machine learning,risk assessment},
publisher = {SAGE PublicationsSage CA: Los Angeles, CA},
title = {{Fairness in Criminal Justice Risk Assessments}},
year = {2018}
}

@inproceedings{Binns18,
author = {Binns, Reuben},
booktitle = {Conference on Fairness, Accountability and Transparency, FAT 2018},
editor = {Friedler, Sorelle A and Wilson, Christo},
pages = {149--159},
publisher = {PMLR},
series = {Proceedings of Machine Learning Research},
title = {{Fairness in Machine Learning: Lessons from Political Philosophy}},
volume = {81},
year = {2018}
}

@inproceedings{Brown2019,
author = {Brown, Anna and Chouldechova, Alexandra and Putnam-Hornstein, Emily and Tobin, Andrew and Vaithianathan, Rhema},
booktitle = {Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems},
doi = {10.1145/3290605.3300271},
pages = {41:1--41:12},
publisher = {ACM},
series = {CHI '19},
title = {{Toward Algorithmic Accountability in Public Services: A Qualitative Study of Affected Community Perspectives on Algorithmic Decision-making in Child Welfare Services}},
year = {2019}
}

@article{Chouldechova2016,
archivePrefix = {arXiv},
arxivId = {1610.07524},
author = {Chouldechova, Alexandra},
eprint = {1610.07524},
journal = {CoRR},
title = {{Fair prediction with disparate impact: A study of bias in recidivism prediction instruments}},
volume = {abs/1610.0},
year = {2016}
}

@article{Corbett-Davies2018,
archivePrefix = {arXiv},
arxivId = {1808.00023},
author = {Corbett-Davies, Sam and Goel, Sharad},
eprint = {1808.00023},
journal = {CoRR},
title = {{The Measure and Mismeasure of Fairness: A Critical Review of Fair Machine Learning}},
volume = {abs/1808.0},
year = {2018}
}

@article{Crasnow2008,
author = {Crasnow, Sharon},
doi = {10.1007/s11191-006-9069-z},
issn = {0926-7220},
journal = {Science {\&} Education},
number = {10},
pages = {1089--1110},
publisher = {Springer Netherlands},
title = {{Feminist philosophy of science: 'standpoint' and knowledge}},
volume = {17},
year = {2008}
}

@article{Crawford2014,
author = {Crawford, Kate and Schultz, Jason},
journal = {Boston College Law Review},
number = {1},
pages = {93--128},
title = {{Big Data and Due Process: Toward a Framework to Redress Predictive Privacy Harms}},
volume = {55},
year = {2014}
}

@inproceedings{Danks2017,
author = {Danks, David and London, Alex John},
booktitle = {Proceedings of the 26th International Joint Conference on Artificial Intelligence},
isbn = {978-0-9992411-0-3},
pages = {4691--4697},
publisher = {AAAI Press},
series = {IJCAI'17},
title = {{Algorithmic Bias in Autonomous Systems}},
year = {2017}
}

@inproceedings{Dwork2012,
address = {New York, NY, USA},
author = {Dwork, Cynthia and Hardt, Moritz and Pitassi, Toniann and Reingold, Omer and Zemel, Richard},
booktitle = {Proceedings of the 3rd Innovations in Theoretical Computer Science Conference},
doi = {10.1145/2090236.2090255},
isbn = {978-1-4503-1115-1},
pages = {214--226},
publisher = {ACM},
series = {ITCS '12},
title = {{Fairness Through Awareness}},
year = {2012}
}

@book{Epp2014,
address = {Chicago},
author = {Epp, Charles R. and Maynard-Moody, Steven and Haider-Markel, Donald P.},
publisher = {University of Chicago Press},
title = {Pulled over: how police stops define race and citizenship},
year = {2014}
}

@book{Eubanks2018,
address = {New York},
author = {Eubanks, Virginia},
isbn = {9781250074317},
pages = {260},
publisher = {St. Martin's Press},
title = {{Automating inequality: how high-tech tools profile, police, and punish the poor}},
year = {2018}
}

@article{Farrelly2007,
author = {Colin Farrelly},
title ={Justice in Ideal Theory: A Refutation},
journal = {Political Studies},
volume = {55},
number = {4},
pages = {844-864},
year = {2007}
}

@article{Feinberg1973,
author = {Feinberg, Joel},
doi = {10.2307/2025007},
journal = {Journal of Philosophy},
number = {9},
pages = {263--275},
publisher = {Journal of Philosophy, Inc.},
title = {{Duty and Obligation in the Non-Ideal World}},
volume = {70},
year = {1973}
}

@article{Feinberg1974,
author = {Feinberg, Joel},
doi = {10.2307/2183696},
journal = {The Philosophical Review},
number = {3},
pages = {297},
title = {Noncomparative Justice},
volume = {83},
year = {1974}
}

@book{Feinberg2014,
address = {Princeton},
author = {Feinberg, Joel},
publisher = {Princeton University Press},
title = {{Rights, Justice, and the Bounds of Liberty: Essays in Social Philosophy}},
year = {2014}
}

@inproceedings{Feldman2015,
address = {New York, NY, USA},
author = {Feldman, Michael and Friedler, Sorelle A and Moeller, John and Scheidegger, Carlos and Venkatasubramanian, Suresh},
booktitle = {Proceedings of the 21th ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
doi = {10.1145/2783258.2783311},
isbn = {978-1-4503-3664-2},
pages = {259--268},
publisher = {ACM},
series = {KDD '15},
title = {{Certifying and Removing Disparate Impact}},
year = {2015}
}

@book{Feldman2016,
address = {Oxford},
author = {Feldman, Fred},
doi = {10.1093/acprof:oso/9780198782988.001.0001},
isbn = {9780198782988},
publisher = {Oxford University Press},
title = {{Distributive Justice}},
year = {2016}
}

@article{Freeman2011,
author = {Freeman, Jonathan B. and Penner, Andrew M. and Saperstein, Aliya and Scheutz, Matthias and Ambady, Nalini},
doi = {10.1371/journal.pone.0025107},
editor = {Gilbert, Sam},
issn = {1932-6203},
journal = {PLoS ONE},
mendeley-groups = {AI fairness},
number = {9},
pages = {e25107},
publisher = {Public Library of Science},
title = {{Looking the Part: Social Status Cues Shape Race Perception}},
volume = {6},
year = {2011}
}


@article{Galston2010,
author = {Galston, William A},
doi = {10.1177/1474885110374001},
journal = {European Journal of Political Theory},
number = {4},
pages = {385--411},
title = {{Realism in political theory}},
volume = {9},
year = {2010}
}

@inproceedings{Glymour2019,
address = {New York, NY, USA},
author = {Glymour, Bruce and Herington, Jonathan},
booktitle = {Proceedings of the Conference on Fairness, Accountability, and Transparency},
doi = {10.1145/3287560.3287573},
isbn = {978-1-4503-6125-5},
pages = {269--278},
publisher = {ACM},
series = {FAT* '19},
title = {{Measuring the Biases That Matter: The Ethical and Casual Foundations for Measures of Fairness in Algorithms}},
year = {2019}
}

@inproceedings{Grgic-Hlaca2018a,
author = {Grgi{\'{c}}-Hlaca, Nina and Zafar, Muhammad Bilal and Gummadi, Krishna P and Weller, Adrian},
booktitle = {Proceedings of the Thirty-Second AAAI Conference on Artificial Intelligence, 2018},
editor = {McIlraith, Sheila A and Weinberger, Kilian Q},
pages = {51--60},
publisher = {AAAI Press},
title = {{Beyond Distributive Fairness in Algorithmic Decision Making: Feature Selection for Procedurally Fair Learning}},
year = {2018}
}

@book{Harding2015,
address = {Chicago},
author = {Harding, Sandra},
publisher = {University of Chicago Press},
title = {{Objectivity and Diversity: Another Logic of Scientific Research}},
year = {2015}
}

@incollection{Hardt2016,
author = {Hardt, Moritz and Price, Eric and Srebro, Nathan},
booktitle = {Advances in Neural Information Processing Systems 29},
editor = {Lee, D D and Sugiyama, M and Luxburg, U V and Guyon, I and Garnett, R},
eprint = {1610.02413},
pages = {3315--3323},
title = {{Equality of Opportunity in Supervised Learning}},
year = {2016}
}

@book{Hellman2008,
address = {Cambridge},
author = {Hellman, Deborah},
isbn = {9780674060296},
pages = {205},
publisher = {Harvard University Press},
title = {{When is discrimination wrong?}},
year = {2008}
}

@article{Hoffmann2019,
author = {Hoffmann, Anna Lauren},
doi = {10.1080/1369118X.2019.1573912},
journal = {Information Communication and Society},
keywords = {Big data,algorithms,antidiscrimination,intersectionality,social justice},
number = {7},
pages = {900--915},
publisher = {Routledge},
title = {{Where fairness fails: data, algorithms, and the limits of antidiscrimination discourse}},
volume = {22},
year = {2019}
}

@techreport{IEEE,
author = {The IEEE Global Initiative on Ethics of
Autonomous and Intelligent Systems},
title = {{Ethically Aligned Design: A Vision for Prioritizing Human Well-being with Autonomous and Intelligent Systems, Version 2}},
year = {2017}
}

@article{Judge2004,
author = {Judge, Timothy A. and Cable, Daniel M.},
doi = {10.1037/0021-9010.89.3.428},
issn = {1939-1854},
journal = {Journal of Applied Psychology},
number = {3},
pages = {428--441},
title = {{The Effect of Physical Height on Workplace Success and Income: Preliminary Test of a Theoretical Model.}},
volume = {89},
year = {2004}
}

@article{Jung2019,
archivePrefix = {arXiv},
arxivId = {1905.10660},
author = {Jung, Christopher and Kearns, Michael and Neel, Seth and Roth, Aaron and Stapleton, Logan and Wu, Zhiwei Steven},
eprint = {1905.10660},
title = {{Eliciting and Enforcing Subjective Individual Fairness}},
year = {2019}
}

@article{Kamiran2012,
author = {Kamiran, Faisal and Calders, Toon},
doi = {10.1007/s10115-011-0463-8},
journal = {Knowledge and Information Systems},
number = {1},
pages = {1--33},
title = {Data preprocessing techniques for classification without discrimination},
volume = {33},
year = {2012}
}

@inproceedings{Kilbertus2017,
archivePrefix = {arXiv},
arxivId = {1706.02744},
author = {Kilbertus, Niki and Rojas-Carulla, Mateo and Parascandolo, Giambattista and Hardt, Moritz and Janzing, Dominik and Sch{\"{o}}lkopf, Bernhard},
booktitle = {Advances in Neural Information Processing Systems},
eprint = {1706.02744},
pages = {656--666},
title = {{Avoiding Discrimination through Causal Reasoning}},
year = {2017}
}

@inproceedings{Kleinberg2017,
author = {Kleinberg, Jon M and Mullainathan, Sendhil and Raghavan, Manish},
booktitle = {Innovations in Theoretical Computer Science Conference (ITCS)},
title = {{Inherent Trade-Offs in the Fair Determination of Risk Scores}},
volume = {67},
year = {2017}
}

@inproceedings{Lipton2018,
author = {Lipton, Zachary C. and Chouldechova, Alexandra and McAuley, Julian},
booktitle = {Advances in Neural Information Processing Systems (NIPS)},
pages = {8136--8146},
title = {{Does Mitigating ML's Impact Disparity Require Treatment Disparity?}},
year = {2018}
}

@article{Liu2018,
archivePrefix = {arXiv},
arxivId = {1803.04383},
author = {Liu, Lydia T. and Dean, Sarah and Rolf, Esther and Simchowitz, Max and Hardt, Moritz},
eprint = {1803.04383},
title = {{Delayed Impact of Fair Machine Learning}},
year = {2018}
}

@article{Mallon2006,
author = {Mallon, Ron},
doi = {10.1086/500495},
issn = {0014-1704},
journal = {Ethics},
number = {3},
pages = {525--551},
publisher = { The University of Chicago Press },
title = {{'Race': Normative, Not Metaphysical or Semantic}},
volume = {116},
year = {2006}
}

@incollection{Miller2017,
author = {Miller, David},
booktitle = {The Stanford Encyclopedia of Philosophy},
edition = {Fall 2017},
editor = {Zalta, Edward N},
howpublished = {$\backslash$url{\{}https://plato.stanford.edu/archives/fall2017/entries/justice/{\}}},
mendeley-groups = {AI fairness},
publisher = {Metaphysics Research Lab, Stanford University},
title = {{Justice}},
year = {2017}
}

@book{Mills1998,
address = {Ithaca},
author = {Mills, Charles W.},
isbn = {0801484715},
publisher = {Cornell University Press},
title = {{Blackness visible: essays on philosophy and race}},
year = {1998}
}

@article{Mills2005,
author = {Mills, Charles Wade},
journal = {Hypatia},
number = {3},
pages = {165--183},
title = {{"Ideal Theory" as Ideology}},
volume = {20},
year = {2005}
}

@article{Montague1980,
author = {Montague, Phillip},
doi = {10.2307/2219277},
issn = {00318094},
journal = {The Philosophical Quarterly},
mendeley-groups = {AI fairness},
number = {119},
pages = {131},
title = {{Comparative and Non-Comparative Justice}},
volume = {30},
year = {1980}
}

@book{Morrison2015,
address = {New York},
author = {Morrison, Margaret},
publisher = {Oxford University Press},
title = {{Reconstructing Reality: Models, Mathematics, and Simulations}},
year = {2015}
}

@article{Nabi2018,
author = {Nabi, Razieh and Shpitser, Ilya},
issn = {2159-5399},
journal = {Proceedings of the ... AAAI Conference on Artificial Intelligence. AAAI Conference on Artificial Intelligence},
pages = {1931--1940},
pmid = {29796336},
publisher = {NIH Public Access},
title = {{Fair Inference on Outcomes.}},
volume = {2018},
year = {2018}
}

@book{OConnor2019a,
address = {Oxford},
author = {O'Connor, Cailin},
isbn = {9780198789970},
mendeley-groups = {AI fairness},
publisher = {Oxford University Press},
title = {{The Origins of Unfairness}},
year = {2019}
}

@book{Pateman2007,
address = {Cambridge},
author = {Pateman, Carole and Mills, Charles Wade},
publisher = {Polity Press},
title = {{Contract and Domination}},
year = {2007}
}

@article{Penner2008,
author = {Penner, Andrew M and Saperstein, Aliya},
doi = {10.1073/pnas.0805762105},
issn = {1091-6490},
journal = {Proceedings of the National Academy of Sciences of the United States of America},
number = {50},
pages = {19628--30},
pmid = {19064936},
publisher = {National Academy of Sciences},
title = {{How social status shapes race.}},
volume = {105},
year = {2008}
}

@article{Petersen1976,
author = {Petersen, Nancy S. and Novick, Melvin R.},
journal = {Journal of Educational Measurement},
mendeley-groups = {AI fairness},
number = {1},
pages = {3--29},
title = {{An Evaluation of Some Models for Culture-Fair Selection}},
volume = {13},
year = {1976}
}

@incollection{Phillips2017,
author = {Phillips, Katherine W.},
booktitle = {The Diversity Bonus: How Great Teams Pay off in the Knowledge Economy},
pages = {223--245},
title = {{What is the Real Value of Diversity in Organizations? Questioning our Assumptions}},
year = {2017}
}

@book{Proctor2008,
address = {Stanford},
author = {Proctor, Robert N. and Schiebinger, Londa},
publisher = {Stanford University Press},
title = {{Agnotology: The Making and Unmaking of Ignorance}},
year = {2008}
}

@book{Rawls1999,
address = {Cambridge},
author = {Rawls, John},
publisher = {Harvard University Press},
title = {{A Theory of Justice}},
year = {1999}
}

@book{Rawls2001,
address = {Cambridge},
author = {Rawls, John},
editor = {Kelly, Erin},
publisher = {Harvard University Press},
title = {{Justice as Fairness: A Restatement}},
year = {2001}
}

@book{Ray1998,
address = {Princeton},
author = {Ray, Debraj.},
isbn = {0691017069},
publisher = {Princeton University Press},
title = {{Development economics}},
year = {1998}
}

@article{Rudolph2009,
author = {Rudolph, Cort W. and Wells, Charles L. and Weller, Marcus D. and Baltes, Boris B.},
doi = {10.1016/J.JVB.2008.09.008},
journal = {Journal of Vocational Behavior},
number = {1},
pages = {1--10},
publisher = {Academic Press},
title = {A meta-analysis of empirical studies of weight-based bias in the workplace},
volume = {74},
year = {2009}
}

@article{Schapiro2003,
author = {Schapiro, Tamar},
doi = {10.5840/jphil2003100727},
journal = {Journal of Philosophy},
number = {7},
pages = {329--355},
title = {{Compliance, Complicity, and the Nature of Nonideal Conditions}},
volume = {100},
year = {2003}
}

@article{Schelling1971,
  title={Dynamic models of segregation},
  author={Schelling, Thomas C},
  journal={Journal of mathematical sociology},
  volume={1},
  number={2},
  pages={143--186},
  year={1971},
  publisher={Taylor \& Francis}
}

@inproceedings{Selbst2019,
 author = {Selbst, Andrew D. and Boyd, Danah and Friedler, Sorelle A. and Venkatasubramanian, Suresh and Vertesi, Janet},
 title = {Fairness and Abstraction in Sociotechnical Systems},
 booktitle = {Proceedings of the Conference on Fairness, Accountability, and Transparency},
 series = {FAT* '19},
 year = {2019},
 isbn = {978-1-4503-6125-5},
 location = {Atlanta, GA, USA},
 pages = {59--68},
 numpages = {10},
 doi = {10.1145/3287560.3287598},
 acmid = {3287598},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {Fairness-aware Machine Learning, Interdisciplinary, Sociotechnical Systems},
}

@article{Sen2006,
author = {Sen, Amartya},
doi = {10.5840/jphil2006103517},
journal = {Journal of Philosophy},
number = {5},
pages = {215--238},
title = {{What Do We Want from a Theory of Justice?}},
volume = {103},
year = {2006}
}

@book{Sen2009,
address = {Cambridge},
author = {Sen, Amartya},
publisher = {Harvard University Press},
title = {{The Idea of Justice}},
year = {2009}
}

@article{Simmons2010,
author = {Simmons, A. John},
doi = {10.1111/j.1088-4963.2009.01172.x},
issn = {00483915},
journal = {Philosophy {\&} Public Affairs},
mendeley-groups = {AI fairness},
number = {1},
pages = {5--36},
title = {{Ideal and Nonideal Theory}},
volume = {38},
year = {2010}
}

@article{Steel2017,
author = {Steel, Daniel},
doi = {10.1007/s10670-016-9859-x},
journal = {Erkenntnis},
mendeley-groups = {AI fairness},
number = {5},
pages = {1065--1084},
publisher = {Springer Netherlands},
title = {{Sustainability and the Infinite Future: A Case Study of a False Modeling Assumption in Environmental Economics}},
volume = {82},
year = {2017}
}


@article{Steel2019,
author = {Steel, Daniel and Fazelpour, Sina and Crewe, Bianca and Gillette, Kinley},
doi = {10.1007/s11229-019-02108-w},
issn = {0039-7857},
journal = {Synthese},
title = {{Information elaboration and epistemic effects of diversity}},
year = {2019}
}

@incollection{Stemplowska2012,
address = {Oxford},
author = {Stemplowska, Zofia and Swift, Adam},
booktitle = {The Oxford Handbook of Political Philosophy},
doi = {10.1093/oxfordhb/9780195376692.013.0020},
editor = {Estlund, David},
pages = {373--389},
publisher = {Oxford University Press},
title = {{Ideal and Nonideal Theory}},
year = {2012}
}

@article{Tuana2010,
author = {Tuana, Nancy},
doi = {10.1007/s11229-010-9793-4},
issn = {0039-7857},
journal = {Synthese},
mendeley-groups = {Thesis},
number = {3},
pages = {471--492},
publisher = {Springer Netherlands},
title = {{Leading with ethics, aiming for policy: new opportunities for philosophy of science}},
volume = {177},
year = {2010}
}

@article{Valentini2012,
author = {Valentini, Laura},
doi = {10.1111/j.1747-9991.2012.00500.x},
journal = {Philosophy Compass},
number = {9},
pages = {654--664},
title = {{Ideal vs. Non-ideal Theory: A Conceptual Map}},
volume = {7},
year = {2012}
}

@article{Woodward2006,
author = {Woodward, James},
doi = {10.1080/13501780600733376},
journal = {Journal of Economic Methodology},
number = {2},
pages = {219--240},
publisher = {Taylor {\&} Francis},
title = {{Some varieties of robustness}},
volume = {13},
year = {2006}
}

@article{Woolley2010,
author = {Woolley, Anita Williams and Chabris, Christopher F and Pentland, Alex and Hashmi, Nada and Malone, Thomas W},
doi = {10.1126/science.1193147},
journal = {Science (New York, N.Y.)},
number = {6004},
pages = {686--8},
pmid = {20929725},
publisher = {American Association for the Advancement of Science},
title = {{Evidence for a collective intelligence factor in the performance of human groups.}},
volume = {330},
year = {2010}
}

@article{Woolley2015,
author = {Woolley, Anita Williams and Aggarwal, Ishani and Malone, Thomas W.},
doi = {10.1177/0963721415599543},
issn = {0963-7214},
journal = {Current Directions in Psychological Science},
number = {6},
pages = {420--424},
title = {{Collective Intelligence and Group Performance}},
volume = {24},
year = {2015}
}

@incollection{Wylie2011,
address = {Dordrecht},
author = {Wylie, Alison},
booktitle = {Feminist Epistemology and Philosophy of Science},
doi = {10.1007/978-1-4020-6835-5_8},
editor = {Grasswick, Heidi E.},
mendeley-groups = {AI fairness},
pages = {157--179},
publisher = {Springer Netherlands},
title = {{What Knowers Know Well: Women, Work and the Academy}},
url = {http://link.springer.com/10.1007/978-1-4020-6835-5{\_}8},
year = {2011}
}

@inproceedings{Zafar2017,
author = {Zafar, Muhammad Bilal and Valera, Isabel and {Gomez Rodriguez}, Manuel and Gummadi, Krishna P},
booktitle = {Proceedings of the 26th International Conference on World Wide Web},
doi = {10.1145/3038912.3052660},
isbn = {978-1-4503-4913-0},
pages = {1171--1180},
publisher = {International World Wide Web Conferences Steering Committee},
series = {WWW '17},
title = {{Fairness Beyond Disparate Treatment {\&} Disparate Impact: Learning Classification Without Disparate Mistreatment}},
year = {2017}
}

@misc{ibm360fairness, 
    title={AI Fairness 360 Open Source Toolkit}, 
    url={https://aif360.mybluemix.net/}, 
} 

@misc{pymetrics, 
    title={Matching talent to opportunity}, 
    url={https://www.pymetrics.com/employers/}
} 

@book{pearl2009causality,
  title={Causality},
  author={Pearl, Judea},
  year={2009},
  publisher={Cambridge university press}
}

@article{liu2018delayed,
  title={Delayed impact of fair machine learning},
  author={Liu, Lydia T and Dean, Sarah and Rolf, Esther and Simchowitz, Max and Hardt, Moritz},
  journal={arXiv preprint arXiv:1803.04383},
  year={2018}
}


==> preamble.tex <==
\usepackage{aaai}
\usepackage{times}
\usepackage{helvet}
\usepackage{courier}
\frenchspacing
\setlength{\pdfpagewidth}{8.5in}
\setlength{\pdfpageheight}{11in}

%\usepackage[utf8]{inputenc}
%\usepackage[letterpaper]{geometry}
%\usepackage[parfill]{parskip}
\usepackage{caption}
\usepackage{subcaption}

%\usepackage[american]{babel}
%eprint = false gets rid of arxiv ids
%\usepackage[backend=biber,style=apa, sortcites=true,doi=false, url=false,isbn=false,eprint=false]{biblatex}
%\usepackage[backend=biber,style=authoryear, sortcites=true,doi=false, url=false,isbn=false,maxnames=2,eprint=false]{biblatex}
% uniquelist=false in biblatex in cases where the second author is not the same / maxcitenames=1
%\DeclareLanguageMapping{american}{american-apa}
%\setlength{\bibitemsep}{0.07in}

\usepackage{amsthm, amssymb, amsmath, latexsym, amsfonts, mathcomp}
\usepackage{xfrac}
\usepackage{verbatim}
\usepackage{color}
\usepackage{mathrsfs}
\usepackage{listings}
\usepackage{enumitem}
\usepackage{array}
\usepackage{url}
\usepackage{footnote}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{fancyhdr}
% \usepackage{natbib}
%\usepackage{libertine}
%\usepackage{libertinust1math}
%\usepackage[T1]{fontenc}
\usepackage[bottom]{footmisc}
\usepackage{float}
\usepackage{algorithm}
\usepackage{algpseudocode}
%\usepackage[noend]{algpseudocode}

\usepackage{setspace}

\makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother

\usepackage[colorlinks=true, linkcolor=black,
            citecolor=black, urlcolor=black,
            bookmarks=true,
            bookmarksnumbered=true,
]{hyperref}

\usepackage{csquotes}


==> sections/causality.tex <==

The causal fairness literature has largely been driven through the lens of Pearl's structural causal models \cite{Pearl2009}. The core idea of causal and counterfactual approaches is that algorithmic unfairness can be seen as the presence of harmful causal influence of protected attributes $A$ on prediction $\hat{Y}$. The approaches differ on whether they take all or some effects of $A$ on $\hat{Y}$ to be harmful as well as whether the effect is framed in terms of population-level interventional or individual-level counterfactual quantities. Below we review three kinds of approaches that frame the discussion of fairness in causal or counterfactual terms.

\subsection{Fair Average Causal Effect}
%%%%%%%%%%%%%%%%%%%% Subsection begins
Consider the design of resume studies aimed at experimentally investigating potential discrimination in academia and hiring \cite{Rooth2010,Moss-Racusin2012}. In a typical study, potential employers receive resumes that are matched in all respect except for applicants' names. Hiring practices are deemed discriminatory when, on average, bearing a name with associations to a disadvantaged group negatively impacts an application's chances of success. In the same vein, some have argued that a classifier is fair if, on average, protected attributes exert no causal influence on the classifier's predictions \cite{Kilbertus2017}. Put in terms of the notion of  ``average causal effect" \cite{Pearl2016}, a classifier is taken to be fair when
\begin{align*}
		P(\hat{Y}=1\mid do(A=a)) - P(\hat{Y}=1\mid do(A=a')) = 0	
\end{align*} 
where the $do$-operator formally represents the notion of a hypothetical intervention, with $do(A=a)$ and $do(A=a')$ indicating ideal interventions setting an individual's protected class to $A=a$ and $A=a'$, respectively. Addressing concerns that interventions on non-manipulable features are conceptually ill-defined \cite{Holland1986,VanderWeele2014}, some papers additionally incorporate a notion of manipulable proxies mediating the worrisome influence of the protected feature \cite{Kilbertus2017}. 

\subsection{Individual Fairness}
%%%%%%%%%%%%%%%%%%%% Subsection begins
Insofar as unfair and discriminatory practices impact \emph{individuals}, one may think that detecting discrimination requires evaluating the way in which an individual's membership to a marginalized group impacted how she was treated. Put another way, one may wish to know how that individual would have been treated had she belonged to a socially dominant group. Indeed, law makers formulate what they take to be the central question of employment discrimination in terms of potential impact on individuals – ``whether the employer would have taken the same action had the employee been of a different race (age, sex, religion, national origin, etc.) and everything else had remained the same” (Carson v. Bethlehem Steel Corp. 82 F .3d 157 159 (7th Circ. 1996)). 

Following this legal definition, some seek to define fairness in terms of counterfactuals pertaining to individuals \cite{Kusner2017,Loftus2018}. Framed in terms of the so-called ``effect of treatment on the treated" formula, a classifier is fair, from this perspective, if
\begin{align*} \label{eq: ETT}
		P(\hat{Y}(a') = y \mid A=a) - P(\hat{Y}(a) = y \mid A=a) = 0	
\end{align*}
where $\hat{Y}(a')$ refers to the value $\hat{Y}$ would take, had $A$ been $a'$, perhaps contrary to the fact. The equation above can be interpreted as requiring that, all else equal, individuals belonging to a protected group should see no change in the decision that was actually made about them, had they belonged to another group. 

\subsection{Path-Specific Illicit Effects}
%%%%%%%%%%%%%%%%%%%% Subsection begins

The phrase ``all else equal" in the individual fairness definition captures the idea that in assessing the counterfactual query of interest the only things that could change are the downstream consequences of the hypothetical alteration to $A$. In graph theoretic terms, we need to keep fixed the non-descendants of $A$, while allowing the set of attributes mediating $A$'s influence on $\hat{Y}$ to vary \cite{Woodward2003a,Pearl2009}. Consequently, the individual fairness criterion can be seen as casting doubt on the fairness of classifiers that permit $A$ to influence $\hat{Y}$ through \emph{any} pathway.\footnote{Whether the criterion casts doubt or automatically labels as unfair depends on whether it is seen as a sufficient condition for algorithmic fairness or as a necessary and sufficient one.} 

\iffalse
\begin{figure}[H]
	\centering
	\includegraphics[clip, trim=0cm 18.75cm 0cm 3.25cm, scale=0.7]{figures/path-specific.pdf}	
	\caption{Disaggregating the sources of variation between two variables.}
	\label{fig:path-specific}
\end{figure}
\fi

Nonetheless, in some contexts, it is admissible and in fact desirable to allow $A$ to causally influence $\hat{Y}$ along certain pathways. This may happen, for example, when a particular characteristic is relevant for a job, even though it is causally related to protected classes. Suppose one culture $a$ values academic discipline $d_a$, while discipline $d_b$  is more prized in culture $b$. Suppose individuals from both cultures put more effort in preparing for the field they value and that as a result they perform better in that field. Intuitively, in this case a classifier whose results vary with group membership may nonetheless be fair, and enforcing individual counterfactual fairness renders the classifier unfair and our intervention paternalistic.

More generally, as highlighted above, we may wish to disaggregate the influence of $A$ on $\hat{Y}$ to better understand the specific \emph{mechanisms} by which $A$ influences $Y$ and to identify the particular pathways of influence that should not be discarded. %Figure \ref{fig:path-specific} depicts the various grains of such a decomposition. 
While individual fairness does not differentiate between distinct ways in which $A$ may influence $\hat{Y}$ and so remains at the level of total effect, others have sought to decompose the overall impact of $A$ into direct and indirect effects, taking such effects to map onto the ethical categories of direct and indirect discrimination  \cite{Zhang2018}. Others have identified fairness as the absence of any effect of protected attributes on the outcome along certain \emph{illicit} pathways, $\pi_1$ \cite{Chiappa2018,Nabi2018}. Such path-specific effects are in turn framed in terms of nested counterfactuals employed in causal literature on mediation \cite{Shpitser2013}.

\section{Shortcomings of Causal Measures} \label{sec:problem-causal}
%%%%%%%%%%%%%%%%%%%% Section begins

Causal approaches provide a powerful way of disentangling different sources of variation between $A$ and $\hat{Y}$, elucidating the reasons for observed associations between the two variables. This is precisely the sort of requisite understanding that statistical measures were incapable of providing. To be sure, causal approaches to framing the question of fairness are more demanding in comparison to statistical measures. For while statistical measures only require the distribution $P(Y,\hat{Y},A,X)$, assessing the causal and counterfactual criteria requires substantial expertise for formulating plausible assumptions regarding the causal structure of the domain of interest. In certain cases, the required causal or counterfactual effects are not identifiable through statistical or even experimental data, unless one makes substantial additional untested and sometimes untestable assumptions \cite{Pearl2009}. One may thus worry about the plausibility of such assumptions and suspect the robustness of the effects identified by these measures. While these worries can be legitimate, one should appreciate the type of transparency provided by causal approaches about where and when a given effect is not identifiable from statistical data and what sort of assumptions are needed to make estimation possible. Indeed, this transparency can be seen as an additional benefit of causal approaches over statistical ones, insofar as it raises novel questions regarding the ethical permissibility of automation in contexts where the requisite causal effects are not identifiable. 

Causal and counterfactual approaches also raise unique conceptual and interpretative challenges that do not arise with statistical measures. Some of these difficulties such as disputes over the causal status of non-manipulable attributes like gender and race are well-known and have been extensively discussed in literature on causality \cite{Glymour2014,Morgan2014}. A typical answer to the worry about manipulability is that some of the various proxies on the path from $A$ to $Y$ are in fact manipulable. And these can be used to investigate questions of discrimination. For instance, in investigating potential discrimination in hiring one may manipulate gender by intervening on ``perception of gender" and examining its effect on hiring decisions. This is the type of answer highlighted in works on causal measures of algorithmic fairness  \cite{Kusner2017,Kilbertus2017}. However, part of the plausibility of answers invoking the use of proxies such as \emph{perception} of protected attributes stems is that the concept of direct discrimination is closely tied to the \emph{mental state} of the discriminator \cite{Altman2016}. 

\par Things get markedly more complicated when we consider broader harms in the context of algorithmic decision making. Specifically for causal approaches, the challenge lies in selecting variables that can meaningfully stand in causal relations. \citeauthor{Kusner2017}, for example, discuss causal models whose variables include a variable, $A$, corresponding to race and a latent variable, $U$, representing ``the totality of socioeconomic factors and policing practices that both influence where an individual may live and how likely they are to be arrested and charged" (p. 4). The problem here is that it is not at all clear that $A$ and $U$ do not overlap, perhaps even \emph{analytically}. Putting aside the challenge of understanding the concept of race \cite{Mills1998,Mallon2006}, this is true even if all that is meant by race is self-identified race. For as research in psychology and sociology show racial classification and identification are shaped by a variety of socio-economic factors \cite{Epp2014,Penner2008}. Such overlaps and dependencies raise two issues for causal approaches: first, if the overlap exists between a protected attribute, $A$,  and another measured variable, $Z$, then due to redundant measurements the two variables become deterministic functions of one another. Causal approaches should thus clarify the conditions under which one can make reliable inferences about the presence of discrimination by manipulating on $A$ (or $Z$). Second, unless $A$ and $Z$ are properly conceptualized, we may be dealing with a situation in which the protected attribute is a compound variable that is both a cause and an effect of $Z$, undermining the reliability of the causal model for inference. These issues reveal the importance of careful \emph{variable choice} -- a task that arguably requires substantial social scientific expertise. 

A further conceptual issue concerns backtracking counterfactuals. For example, from unfair grading to prejudiced assessments of their academic potentials, students with immigrant backgrounds face a range of injustices throughout their education \cite{Bonefeld2018,Kiss2013}. If they also have an accent that is more negatively evaluated than others, they are further disadvantaged by decisions in hiring and promotion contexts \cite{Huang2013,Chin2009}. Focusing on hiring decisions, such individuals would have plausibly received more favourable treatments, if they were of a different ethnic origin. But how should we interpret a counterfactual involving a hypothetical change to someone's ethnic origins in a way that is \emph{non-backtracking} -- without changing factors about that individual \emph{prior} to the hypothetical change. Furthermore, how can we interpret this hypothetical intervention in a way that does not alter other task-relevant facts about the individual (e.g., school names, extra-curricular activities, languages spoken, ...) that could potentially impact the outcome of interest via distinct causal pathways. Similar points apply to changing someone's race and gender. What is needed is clarity regarding the type of manipulation that is relevant to our inferential goals. To my knowledge, causal and counterfactual measures of fairness leave these questions unanswered. Yet, noting these issues is crucial insofar as fairness assessment tools should provide the end user of the tool with clear advice about what is required to make the tool operative in a particular context.

Let us now consider the set of desiderata more broadly. The causal approaches thus far proposed fail to address many of the core problems for which they were regarded as a panacea. To begin, current work relies as heavily as its statistical antecedents on the specification of protected attributes $A$, and although they often invoke the idea of procedural fairness \cite{Zhang2018}, they address only the aspect of procedural fairness concerning the protected features. No approach that we have encountered identifies unfairness more generally in its comparative and non-comparative guises. For instance, causal definitions of fairness would not hold it to be unfair to grant loans or parole on the basis of some extraneous factors, unless the factor sat on the causal pathway between $A$ and $\hat{Y}$. Furthermore, even with respect to the specified protected attributes, counterfactual and causal approaches have the undesirable property of being anonymous and insensitive to the particular labeling of groups with different sensitive attributes. They thus raise false alarms in cases where the influence of the protected attribute on predictions is not morally objectionable. For example, we might hope that a mature causal theory of fairness could distinguish between the the mechanism by which disparities between black and white Americans emerged (via centuries of slavery, segregation, and denied educational and economic opportunities) compared to those by which Americans of east Asian descent appear advantaged (not through any systemic discrimination against whites) \cite{Hartocollis2017}. However, in both cases, the counterfactual fairness approaches would require treatment parity, in one case righting a historical wrong, and in the other compounding current discrimination.

As they stand, therefore, causal approaches miss non-comparative harms as well as the morally relevant asymmetries that make anonymity an undesirable property of metrics of comparative harms. One may suggest that the morally relevant asymmetries could be detected if causal structures were extended back in time to encompass the relevant historical factors that distinguish the cases. This only serves to highlight the more general point, however: \emph{unless} we already believe that \emph{there is} some morally relevant asymmetry there waiting to be discovered, we would not expand the causal structure. By themselves, causal and counterfactual approaches are silent on what is the \emph{relevant} causal structure from an ethical point of view. Even given the relevant structure, the direct use of $A$ in calculating $\hat{Y}$ is relatively easy to detect. The ethical nature of the indirect influence of $A$ on $\hat{Y}$, however, accounts for nearly all of the practical difficulty in addressing issues of fairness. While some approaches (e.g., \citeauthor{Nabi2018}) are cognizant of this challenge and are commendably explicit about their reliance on exogenous guidance for distinguishing between worrisome and admissible pathways, the vast majority of current approaches evade the questions of \emph{how to determine} which pathways are ethically problematic. 

\par This issue can be framed using the construct of a fair possible world: the causal approaches proposed thus far take the specification of a fair counterfactual world, where $A$ does not have a (worrisome) causal impact on $\hat{Y}$, as a given. Equipped with tools of causal inference, they seek to detect potential differences between what happens in the \emph{actual world} and what would have happened in this \emph{fair possible world}. Yet, the core challenge in fairness assessment stems from identifying what counts as the relevant fair world. Consider, for instance, different ways in which a fair world might be conceptualized on a grand scale: it may be tempting to think of such a world as a future-oriented ideal state of affairs in which ``our" values are realized. Adopting a historical perspective, on the other hand, it may be argued that the fair alternative is one that would have arisen had our social institutes arisen justly \cite{Bader2017}. While these two conceptions of ideal possibilities -- prospective and historical -- overlap, they can also come apart. To add to the difficulty, each possibility can in turn be specified in a multitude of ways, subject to a host of value disagreements. The range of  possibilities generate substantive complexities in determining the ethically relevant causal structure, the ethically relevant pathways within that structure, and, indeed, the ethically permissible range of influence relayed through those pathways.

Even with all the relevant information in hand, complications arise with respect to the question of \emph{whether} and if so \emph{how} one should correct for worrisome influences of $A$ and $\hat{Y}$. Take, for instance, the claim that, under certain conditions, demographically diverse groups can outperform homogeneous groups \cite{Woolley2010,Phillips2017,Steel2018}. A number of different, though often complementary, mechanisms have been postulated to explain this positive effect of diversity on group performance. According to some, whereas members of dominant groups often tacitly accept the prevailing viewpoints, individuals from marginalized groups are more likely to develop standpoints that lead to novel solutions \cite{Harding2015,Crasnow2008}. According to others, certain interaction styles that tend to be associated with gender socialization, such as those exhibiting emotional intelligence and promoting democratic turn-taking, enhance the integration of information distributed among group members \cite{Bear2011a,Woolley2010}. Notice that both of these explanations rely on mechanisms that arise \emph{as a result of} socially unjust histories. And, yet, it would be unfair to discard the resultant perspectives and abilities that should give the affected individuals unique positions in, say, admission and hiring contexts. 

\par Causal approaches to fairness need to address graphs whose pathways correspond to events potentially unfolding over decades. Causal fairness papers to date address \emph{is there discrimination?} but leave open the questions of \emph{who discriminated?} and \emph{what are the responsibilities of the current decision-maker?} If sensitive features influence education, which in turn influences employment decisions, then to what extent does the causal effect reflect the discrimination of the education system compared to that of the employer? The answer to this question is not straightforward and requires legal expertise. Neglecting this fact, causal approaches often simply combine these effects. While identifying disparities on a grand scale is valuable unto itself, it provides little moral or legal guidance to the decision-maker: while the influence of protected attributes on predictions may reflect injustice, to guide decisions we must identify not only what would constitute a just world but also what constitutes a just decision in the given world. Ultimately, then, insofar as measuring \emph{fairness} goes, causal approaches must rely on exogenous guidance for choosing the set of appropriate variables, the relevant causal structure over the set of variables, the relevant pathways in a given structure, and the relevant range of causal effect.

\section{Designing Fair Predictors} \label{sec:mitigate}
%%%%%%%%%%%%%%%%%%%% Section Begins

To see the far-reaching consequences of the discussion thus far, it is worth connecting our discussion concerning measures of fairness with current work on \emph{mitigating} algorithmic unfairness and designing fair predictors. Overall, there are three types of mitigation strategies. The first strategy builds on the idea that if our dataset does not reflect societal biases, then the model learned from this data will also be untainted. Accordingly, some researchers intervene in the \emph{pre-processing} stage to shape and cleanse the training dataset so as to construct fair representations that can then be fed to learning algorithms \cite{Zemel2013,Kamiran2012}. The second strategy is based on the idea that the patterns learned from a potentially biased dataset may still be fair if one proceeds in a circumspect way. To ensure fairness, the learning process is constrained, for instance, by penalizing models that assign too much weight to sensitive attributes such as race or gender. This approach intervenes in the \emph{learning} stage of model building by modifying the cost function used in optimization \cite{Zafar2017,Celis2019}. The technique thus fits nicely with traditional ways of shaping the cost function such as regularization. 

Finally, specifically in classification tasks, one may see a mitigation opportunity in the gap between belief (e.g., an estimated score) and assertion (e.g., assigning a label). From this perspective, decision making in high stake settings requires higher standards of evidence. This is not unlike our typical practice; given the same degree of certainty, we may feel more comfortable making an assertion amongst friends than in a court. So, intervening in the \emph{post-processing} stage, this strategy involves modifying the utility function governing the relationship between estimated probabilities and predicted labels, sometimes setting different evidential thresholds for different groups \cite{Pleiss2017,Hardt2016}. 

There are different benefits and shortcomings to each of these mitigating strategies. Nonetheless, regardless of the approach, any successful mitigation strategy requires possessing an adequate technique for measuring algorithmic fairness. Mitigation strategies are means towards the goal of constructing fair predictors that are as accurate as possible. Evaluating the success of any mitigation strategy requires an adequate metric that tells us whether that goal has been achieved. Indeed, in the absence of adequate metrics, poorly guided and monitored mitigation techniques can in fact result in harmful unexpected side effects. A useful illustration of this possibility is provided by Lipton et al. \shortcite{Lipton2018} in relation to \emph{disparate learning processes} (DLPs) techniques that seek to jointly satisfy blindness and demographic parity.

The core idea behind DLPs is that protected attributes can be explicitly used during training in order to learn a ``fair classifier”, from the perspective of some demographic parity measure, but not during deployment, thus satisfying blindness \cite{Pedreshi2008,Zafar2017}. This idea can be implemented by intervening in pre-processing (e.g., using preferential sampling) \cite{Kamiran2012} or during learning (e.g., using fairness constraint) \cite{Zafar2017}. In each case, the hope is to reconcile blindness and demographic parity. Despite the initial attraction of these methods, some studies show that DLPs can in fact result in other harms. Imagine a company that wants to automate its hiring procedure. Suppose, decisions about hiring are only based on work experience. But, due to historical reasons, men have more experience than women. Suppose further that men and women also differ with respect to other attributes, such as hair length, that are irrelevant to the target variable. %This set up is depicted in figure \ref{fig:irrelevant-mitigate}. 

%%%%%%%%%%%%%%%%%%%% Model from Lipton et al 2018
\iffalse
\begin{figure}[H]
	\centering
	\includegraphics[clip, trim=5cm 21cm 5cm 3.75cm, scale=0.99]{figures/lipton.pdf}	
	\caption[The toy model of synthetic hiring data]{The toy model used to generate the synthetic data in \cite{Lipton2018}. $G$: gender, $E$: work experience, $L$: hair length, and $H$: hiring. Solid directed edges indicate causal influences.}
	\label{fig:irrelevant-mitigate}
\end{figure}
\fi
%%%%%%%%%%%%%%%%%%%% End figure

As Lipton et al. \cite*{Lipton2018} show, in an attempt to rectify the disparity in hiring due to differential work experience, DLPs achieve parity by giving weight to the irrelevant proxy (hair length). Aside from the non-comparative harm of making hiring decisions on irrelevant grounds, the supposed remedy in fact hurts some short-haired women, while helping some long-haired men. What is more, by incentivizing the possessing of long hair among female applicants, the supposed mitigation strategy also reinforces social stereotypes. Yet, insofar as the two measures of fairness -- blindness and demographic parity -- are concerned the outcome appears fair. In light of such circumstances, therefore, developing more comprehensive means of assessing fairness is all the more pressing. To be sure, it may be that we cannot escape some type of trade-off between different kinds of harms. The point is not that trade-offs between different morally relevant factors can be avoided when mitigation strategies are guided by more comprehensive assessment techniques. Rather, the idea is that with more adequate assessment techniques we at least know \emph{that} some trade-off is being struck and \emph{what} that trade-off is. 

%%%%%%%%%%%%%%%%%%%% General Discussion

\section{General Discussion} \label{sec:discussion}

Guided by the analysis so far, below we make a number of suggestion for making progress on combating harms of algorithmic decision making.

\subsection*{Harms beyond discrimination}
Construction of operative assessment tools is the first step towards effective risk management. Yet, because of their exclusive focus on discriminatory harms, current metrics of algorithmic fairness are insensitive to a host of other comparative and non-comparative injustices. To be sure, there are sensible reasons for paying special heed to the potential of automation to adversely impact historically disadvantaged groups. One may also assume that by default automation eradicates other harms, such as those resulting from decision making on extraneous grounds. Ultimately, however, heightened attention to one type of harm should not lead to a complete neglect of others. In particular, a meaningful \emph{criterion} of fairness cannot operate on the basis of the assumption that these other comparative and non-comparative harms are not going to be present. Indeed, as we have seen, enforcing narrow fairness criteria can itself be a source of harms.

\subsection*{Transparency about the scope of the metrics}
A policymaker glancing at literature on algorithmic fairness is likely to be misled about a number of issues. First, the literature is plagued by the misuse of language; statistical and causal constructs are referred to using terms with substantive ethical and legal significance; conditional and unconditional probabilistic dependence are referred to as disparate treatment and impact; equality of classification sensitivity is seen as invoking equality of opportunity; direct and indirect causal effects are somehow mapped onto direct and indirect discrimination. The unfortunate choice of terminology actively obfuscates the relation between fairness measures and the ethical concepts with the same name, resulting in much confusion on behalf of policymakers and researchers alike \cite{Lipton2018a}. 

More fundamentally, whether statistical or causal, all measures of algorithmic fairness rely on \emph{exogenous} specification of morally relevant cases and classes. Except for a handful of causal approaches, however, there is no explicit admission of this fact. Indeed, statistical measures give rise to the impression that the only ``ethical" input that is needed for assessing algorithmic fairness is the set of protected attributes $A$; statistical constructs are supposed to take care of the rest.\footnote{In the case of some statistical measures, the implicit assumption may be that, given the proprietary nature of many algorithms,  the joint distribution $P(Y, \hat{Y}, A, X)$ is all we could hope to have access to in determining fairness. Estimation is one thing, however, and definition is another. Specifically, worries about what we can and cannot do in estimation should not influence how we define a criterion. Rather, we first define the criterion as best as we can and then think about what we need in estimating the construct.} The situation is unfortunate. This is not only because what counts as morally relevant is given exogenously. But because it is given exogenously by some \emph{individual or organization}. Arguably, this lack of transparency about which values -- belonging to and promoted by whom -- are encoded in measures of fairness goes against the very essence of what research on algorithmic fairness stands for.

\subsection*{From fairness measures to a causal toolbox for diagnosis}
A typical paper on algorithmic fairness starts with a brief description of what fairness is. It then asserts, seldom with much argument, an equivalence between that description and what is often a well-known statistical construct, calling the construct a fairness measure or criterion. The paper ends by proposing an intervention for satisfying the proposed criterion. Especially with statistical measures, this pipeline for constructing allegedly fair predictors \emph{appears} automated. \iffalse The optimistic sentiment behind this sort of effort is nicely expressed by a user on a popular data science and machine learning platform: 
\begin{quote}
	Bias may be a human problem, but amplification of bias is a technical problem -- mathematically explainable and controllable byproduct of the way models are trained. Consequently, mitigation of existing bias is also a technical problem.\footnote{Get rid of the reference %\url{https://towardsdatascience.com/algorithmic-solutions-to-algorithmic-bias-aef59eaf6565}
	}
\end{quote} \fi
\noindent Our close examination of the evolution of fairness metrics casts serious doubts on this type of claim about automatic fairness ``certification".

More generally, going beyond discriminatory harms and accounting for the other comparative and non-comparative harms requires a context-sensitive approach. Non-comparative harms, for example, consist of divergence from normative standards that are relevant given the specifics of the case. It is thus more productive to approach the issue from the perspective of developing a diagnostic toolbox as opposed to a single metric. Tools of causal inference will be part of this toolbox; aside from the promise of mediation analysis in detecting potentially harmful impacts of protected attributes on predictions, causal knowledge is also crucial for determining task relevance, thus contributing to the detection of some non-comparative harms. Moreover, compared to statistical criteria of disparate impact, causal decision theory is arguably a more suitable tool for providing insight about the impact of decisions on different groups. In the context of loan approvals, for example, demographic parity would naively require equal approval rates across different groups, regardless of the long term impact of offering loans to individuals who may be unable to repay it. 

Causal modeling can also prove beneficial with respect to other sources of bias, such as dealing with sampling bias and clarifying the conditions under which the model trained on a particular sample may be generalized to a deployment context of interest \cite{Bareinboim2014,Pearl2014}. What is more, in many cases, the best mitigation strategy may not involve modifying the classifier but instead require changing the social environment in which the classifier operates. Causal modeling can play a larger role in shedding light on potential point of interventions suitable for bringing about more equitable outcomes over time. With respect to each of these potential roles, however, causal tools must be supplemented with substantive amount of expert insight from different disciplines.

Current research seeks to develop tools that ensure that ML-based decision systems yield allocations that are just in an unjust world. Here we have argued that current efforts (1) provide incomplete and misguiding diagnosis, (2) they lead to incomplete and misguided mitigation efforts, (3) they have limited practical utility from the current decision-maker, and (4) that they conceal embedded value judgments. 

==> sections/related.tex <==
\cite{Danks2017,Binns18,Selbst2019,Hoffmann2019,Barabas2018}

==> sections/statistical-measures.tex <==
One set of attempts to develop fairness measurement techniques work in the language of statistics, where the fairness of an algorithmic decision was seen as a property of the joint distribution $P(Y, \hat{Y}, A, X)$ with random variables corresponding to ground truth $Y$, predictions $\hat{Y}$, a subject's protected characteristics $A$ (say race, gender, etc), with values $a$ and $a'$, and their (possibly correlated) other attributes $X$. In this section, we motivate and introduce four distinct statistical measures. We end the section by highlighting a common weakness of all statistical measures.

\subsection{Fairness through Blindness} \label{sec:blindness}
%%%%%%%%%%%%%%%%%%%% Subsection begins

We may think that fairness consists in treating equals equally. Thus, policies or procedures that yield divergent outcomes for individuals who are similar in relevant respects are unfair. Building on this conception of procedural fairness, we may insist that given their \emph{irrelevance}, protected attributes (sex, race, ...) should not make a difference to how individuals are treated, though it is often unclear whether the irrelevance of protected attributes is taken as a matter of how things \emph{actually are} or how they \emph{ought to be}. Some seek to capture this idea by requiring that, given a set of non-protected attributes $X$, protected attributes $A$ should not make a difference to the outcome $\hat{Y}$. In other words,
\begin{align*}
	P(\hat{Y}=1\mid A=a,X=x) = P(\hat{Y}=1\mid A=a',X=x) 
\end{align*}
where $a$ and $a'$ refer to the two classes of a binary protected attribute \cite{Grgic-Hlaca2018a,Qureshi2016}. Some accounts expand $A$ to include proxies for protected attributes. This measure is often seen as related to the disparate treatment doctrine in US labour law prohibiting direct discrimination, and it is often referred to by that name.

\subsection{Demographic Parity} \label{sec:parity}
%%%%%%%%%%%%%%%%%%%% Subsection begins

Depending on the context, procedures that do not explicitly rely on protected attributes may nonetheless be unfair. This is because protected attributes often have a range of seemingly neutral surrogates; our gender, ethnicity, nationality, sexual orientation, economic status and political beliefs can potentially be read off from names, postal codes, the make and model of one's car, the websites one visits, and so on. As amply shown by redlining practices -- denying certain services on the basis of racially associated information such as zip codes -- seemingly neutral surrogates such as postal codes can be used to systematically deny services to members of particular social groups. 
%To see why, consider the U.S. Supreme Court case, \emph{Griggs v. Duke Power}, where the company used written tests to make promotion decisions. The historical inequalities in educational opportunities meant that, despite its neutral appearance, the policy would result in substantial disparities between white and black workers, adversely impacting the latter's chances of promotion. The company's conduct was judged to be \emph{indirectly} discriminatory, since the sort of skills measured by the test could not ``be shown to be related to job performance".\footnote{In general, disparate impact by itself does not suffice for establishing discrimination. While different legal systems vary in terms of what they require for establishing indirect discrimination, the defendants are typically required to show that decisions are made on grounds that are relevant to the goal and are thus justified given the aim. So, a policy that leads to disparate outcomes for different protected classes may be considered lawful, if it can shown that the policy is ``motivated by a legitimate aim and the means are appropriate and necessary to achieve the aim” (\citeauthor[864]{Osin2005} cited in \citeauthor{Altman2016}.} More generally, 

Given these considerations, one may think that a distributive procedure is unfair if its outcome adversely impacts one protected group at a substantially higher rate than another. It is tempting to formalize this idea using some measure of association between sensitive attributes $A$ and the predicted outcome $\hat{Y}$ \cite{Calders2009,Zemel2013,Zafar2017}. For example, we may demand that a fair classifier's predictions should be statistically independent from protected attributes, that is, $\hat{Y} \perp A$. 
\iffalse
% I can summarize the following in terms of some contsraint on risk difference and risk ratio
One can restrict the constraint to \emph{substantial} disparities, by relaxing this independence condition such that
\begin{align}\label{eq:RD}
	\vert P(\hat{Y}=1\mid A=a) - P(\hat{Y}=1\mid A=a')\vert \le \epsilon	
\end{align}
\noindent where the magnitude of $\epsilon$ can vary depending on how the notion of ``substantially" different impact is understood in a given legal context. 

\par The expression on the left hand side of equation \ref{eq:RD} is called ``risk difference". Another measure of association between $A$ and $\hat{Y}$ is the ``risk ratio". Put in terms of risk ratio, a classifier is fair when
\begin{align}\label{eq:RR}
	\frac{P(\hat{Y}=1\mid A=a)}{P(\hat{Y}=1\mid A=a')} \geq \epsilon	
\end{align}
\noindent This metric has been quite popular, since, with $\epsilon$ set to $0.8$, it captures the 80\% test of disparate impact proposed by the US Equal Employment Opportunity Commission \cite{Feldman2015}\footnote{The U.S. EEOC. Uniform guidelines on employee selection procedures, March 2, 1979.}. Indeed, thus specified, the measure is often referred to as ``disparate impact", synonymous with the legal doctrine. 
\fi
\subsection{Equalized Odds}
%%%%%%%%%%%%%%%%%%%% Subsection begins

The criteria considered thus far have operated on the basis of the assumption that the protected attributes and their prima facie neutral proxies are in some way \emph{irrelevant} to the legitimate aims of the distributive procedure, where irrelevance is understood in terms of probabilistic independence. There are many cases in which this assumption does not hold: sex and gender can be relevant to classifications in medical diagnosis. Economic status is relevant to the ability to repay a loan. Eligibility for admission into a particular graduate program may be correlated with one's cultural background. This can happen, for example, if different cultures prize different fields of study. For an example of this sort see \cite{Dwork2012}.

\par One way of translating this idea into the language of statistics is to insist that, while there may be some correlation between a classifier's predictions and protected attributes, the dependency must be ``explained", or more accurately screened off, by the target variable; if we know the value of $Y$, knowing an individual's sensitive attributes should not give us any further information about the classifier's predictions. So, a classifier is fair if
\begin{align*}
	\hat{Y} \perp A \mid Y
\end{align*}
From this perspective, a fair classifier is one that performs equally well for different protected groups, when evaluated with traditional performance measures such as sensitivity and specificity. There are various ways of relaxing the equalized odds criterion, with some only demanding a parity of sensitivity and some a parity of specificity across different groups \cite{Chouldechova2016}. Depending on the particular specification, the criterion has been interpreted in different ways. For example, some have interpreted the demand for equal false negative rates as capturing the ethical and legal notion of \emph{equality of opportunity} \cite{Hardt2016}.
\iffalse
%%%%%%%%%%%%%%%%%%%% Table for equalized odds and calibration
\begin{table}[H]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|ll|l|l|l|}
\hline
\multicolumn{2}{|l|}{\multirow{2}{*}{}} & \multicolumn{2}{c|}{\textbf{Predicted label}} &  \\
\multicolumn{2}{|l|}{} & $\hat{Y}=0$ & $\hat{Y}=1$ & Total \\ \hline
\multicolumn{1}{|c}{\multirow{2}{*}{\textbf{True Label}}} & $Y=0$ & True negative (TN) & False positive (FP) & $N = TN + FP$ \\ \cline{2-5} 
\multicolumn{1}{|c}{} & $Y=1$ & False negative (FN) & True positive (TP) & $P = FN + TP$ \\ \hline
\multicolumn{1}{|l}{} & Total & $N^* = TN + FN$ & $P^* = FP + TP$ &  \\ \hline
\end{tabular}%
}
\caption[Confusion matrix representing classification performance]{A confusion matrix representing classification performance. $P$ and $N$ refer to the total number of actual positive and negative instances in the population, respectively. $P^*$ and $N^*$ refer to total number of instances predicted by the classifier to be positive and negative instances, respectively. The performance of the classifier can be evaluated using metrics based on the quantities in the matrix. The specificity of the classifier (true negative rate), $P(\hat{Y}=0 \mid Y=0)$, is approximated by $\frac{TN}{N}$. Sensitivity (true positive rate, hit or recall), $P(\hat{Y}=1\mid Y=1)$, is given by $\frac{TP}{P}$. Positive predictive value (or precision), $P(Y=1\mid \hat{Y}=1)$, is estimated by $\frac{TP}{P^*}$ and negative predictive value, $P(Y=0\mid \hat{Y}=0)$,  is $\frac{TN}{N^*}$.}
\label{table:confusion-matrix}
\end{table}
\fi
\subsection{Calibration}
%%%%%%%%%%%%%%%%%%%% Subsection begins
There are different performance metrics to choose from when specifying the idea that a fair classifier is one that performs equally well for different protected classes. While equalized odds approaches focus on metrics such as sensitivity and specificity, one may think that parity of predictive power is the relevant metric. According to this view, when a fair classifier \emph{predicts} that a person belongs to a particular class or condition, then the probability that the classification is correct is the same regardless of the individual's protected group membership. Formally
\begin{align*}
	Y \perp A \mid \hat{Y}
\end{align*}
In other words, no further insight should be gained by knowing an individual's class membership, once the classifier's prediction is known. This fairness metric is thus violated by classifiers that exhibit disparate \emph{precision} (or positive predictive value) for different protected classes. Same goes for classifiers that do not have the same negative predictive value across different protected groups. Accordingly, this criterion can be specified with different degrees of strictness depending on whether one requires a parity of positive predictive value, negative predictive value, or both \cite{Kleinberg2017,Dieterich2016}.

%%%%%%%%%%%%%%%%%%%% Section begins
\section{Shortcomings of Statistical Measures} \label{sec:problem-statistical}
Prima facie, statistical criteria appear to be quite transparent in that the joint distribution $P(Y, \hat{Y}, A, X)$ is all they require for assessing a predictor's fairness. Nonetheless, these measures suffer from serious shortcomings. It is easy to conjure scenarios where a classifier would violate common notions of fairness, despite satisfying a given statistical criterion: As mentioned above, in some contexts, blindness might block the very policies required to promote equality \cite{Hardt2016,Corbett-Davies2018}. Demographic parity naively requires equalizing outcomes, even if this results in decisions based on irrelevant features \cite{Lipton2018}, even if the characteristics of interest occur in different frequencies in the two populations \cite{Dwork2012}, and regardless of whether this sort of equality leads to long term harms \cite{Liu2018}. Similarly, among other problems, equalized odds and calibration preserve harmful biases that may be encoded in true labels \cite{Kusner2017}. So, these measures exhibit poor sensitivity. One may think that, while individually inadequate, the criteria can jointly ensure the fairness of classification systems. Many statistical conditions are mutually irreconcilable, however. When two protected groups differ in terms of their population base rate, for example, equalized odds and equalized predictive value cannot be jointly satisfied \cite{Chouldechova2016,Barocas2018}. Moreover, techniques aiming to reconcile blindness with demographic parity may themselves promote other types of harms by incorporating otherwise irrelevant proxies for $A$ \cite{Lipton2018}.

The problem with sensitivity is indicative of a more fundamental problem, however. The complete reliance of statistical measures on the legal specification of the protected attributes seriously limits the diagnostic adequacy of these measures. The set of protected attributes define what the statistical criteria in effect take to be the set of ``morally" relevant contrast classes. Each statistical criterion tests for a particular type of statistical disparity between these exogenously defined contrast classes. Importantly, insofar as the statistical measures are concerned, these disparities \emph{exhaust} the set of potential allocative harms. It is not difficult to see how this can be perilous, however. First, the list of morally relevant contrast classes in a given situation is not exhausted by the legal list of potential grounds of discrimination. Suppose, for example, that the appraisal of an employee's performance is influenced by factors such as their weight or height, despite the irrelevance of such characteristics to the job \cite{Judge2004,Rudolph2009}. A classifier trained on this historical record may thus predict that, regardless of their gender, overweight individuals are not promising job candidates, thus adversely impacting their chances of career advancement. In this setting and from the perspective of comparative justice, height and weight \emph{are} morally relevant categories. Indeed, the relevant contrast classes may be even more case-specific: for example, if grading practices are influenced by extraneous factors such as the font of a piece of writing, then one can contrast essays written in serif with those that are written in non-serif fonts. More generally, if we think some attribute is or should be irrelevant to the outcome, our measure should be sensitive to observed discrepancies between individuals on ground of their status vis-à-vis that attribute. 

What is more, not every morally relevant contrast class is \emph{statistical}. At a broad level, fairness of an allocative procedure is a matter of whether the procedure gives individuals what is their due. As noted by Feinberg \cite*{Feinberg1974}, in some cases, what is someone's due is determinable only in comparison to how others have been treated. In other cases, no comparison is required and an individual's due is determinable independently and by reference to how that individual \emph{should have been} treated according to some independent standard \cite{Feldman2016}. An allocative procedure can thus impose \emph{comparative} as well as \emph{non-comparative} harms on individuals. Suppose, influenced by extraneous factors, a judge treats all defendants equally, denying parole to them all regardless of the specifics of their case. Here the defendants are harmed not because of any actual disparity, but because of a divergence from how they \emph{should have been} treated from the perspective of the standards of retributive justice; the review process was based on legally irrelevant factors, infringing on defendants’ rights to due process, and the punishments, at least in some cases, were disproportionately harsh, given the crime. Due to their focus on a list of legally specified grounds of discrimination, such allocative harms are likely to escape the purview of statistical measures, rendering these measures insensitive to many cases of comparative and non-comparative injustices.

Similar worries arise with respect to the specificity of statistical measures. Statistical measures have the property of being \emph{anonymous} or \emph{symmetric}; according to these measures, whether a distribution of benefits and burdens is fair does not depend on who the affected individuals or groups are. Put in terms of the protected attributes, anonymity says that the fairness of a distribution does not depend on the meaning attached to labels $a$ and $a'$. In certain contexts and for certain purposes, anonymity is a desirable property. Quantitative metrics of \emph{income inequality} are required to be anonymous, for example, because ``from an ethical point of view, it does not matter who is earning the income" \cite{Ray1998}. The same cannot be said about justice and fairness, however, where it matters very much how and on what grounds the benefits and burdens were distributed and who was adversely impacted by that distribution. 

More fundamentally, unlike the case of income inequality, evaluating fairness claims requires going beyond the \emph{observation that} some disparity exists; we need to know \emph{why} the disparity exists and how it came about.\footnote{This point is, of course, well-known from historical cases of discrimination \cite{Cartwright1979,Pearl2016}.} Suppose we observe some disparity between the admission rate of males and females into a graduate school.\footnote{The example is based on the investigation of gender bias in UBC Berkeley's graduate admission \cite{Bickel1975}.} Why is that? It may be that the admission procedure is discriminatory, influenced either directly or indirectly by an applicant's gender. But there are other explanations: it may be that there is a relationship between gender and department choice, such that female applicants for one reason or another tended to apply to more competitive departments. Or, there may be a relation between gender and some admission-relevant characteristic: perhaps unequal educational opportunities created a disparity in knowledge. Perhaps grading practices were biased against female students. Or it may be that male applicants are more favourably appraised by their reference letter writers \cite{Madera2009}. 

%Figure \ref{fig:simpsons} depicts some of these possible answers using a causal graph. 
Depending on how the disparity came about, it may turn out that it is not morally objectionable. In some other cases, we may find the situation morally problematic, but nonetheless think that correcting the injustice is not the responsibility of the graduate school admission system itself (e.g., if the source of grade disparity is very much upstream). And in yet other cases, we may consider the admission system discriminatory. Given their inability to discern the relevant differences between these scenarios, statistical measures afford little guidance to the current user. 

%%%%%%%%%%%%%%%%%%%% Grad admission
\iffalse
\begin{figure}[H]
	\centering
	\includegraphics[clip, trim=5cm 19.6cm 5cm 3.75cm, scale=0.99]{figures/simpsons.pdf}	
	\caption[Potential sources of disparity in graduate school admissions]{Potential sources of disparity in graduate school admissions. $A$: gender, $X_1$: department choice, $X_2$: relevant factors (e.g., grades, reference letters, ...). Solid directed edges indicate causal influences that actually obtain and dashed edges represent potential causal relations that may explain the disparity.}
	\label{fig:simpsons}
\end{figure}
\fi
%%%%%%%%%%%%%%%%%%%% End figure

Questions of fairness, then, are causal questions and investigating them requires refocusing our attention from observed patterns to the underlying causal structures that have generated these patterns. Conceivably, understanding the causal mechanisms giving rise to our data could help us better formulate problems of fairness in the following ways: provide a more general notion of fairness that relies less on the specified groups, and can more generally identify potential distributive harms; tease apart the process by which $A$ became correlated with $Y$, providing guidance on which observed disparities are the responsibility of the present decision-maker. Indeed, a causal perspective can also clarify when and in what contexts the verdicts of a given statistical metric can be trusted, and why.

